FLASH-FHE: A Heterogeneous Architecture for Fully Homomorphic Encryption Acceleration

While many hardware accelerators have recently been proposed to address the inefficiency problem of fully homomorphic encryption (FHE) schemes, none of them is able to deliver optimal performance when facing real-world FHE workloads consisting of a mixture of shallow and deep computations, due primarily to their homogeneous design principle. This paper presents FLASH-FHE, the first FHE accelerator with a heterogeneous architecture for mixed workloads. At its heart, FLASH-FHE designs two types of computation clusters, ie, bootstrappable and swift, to optimize for deep and shallow workloads respectively in terms of cryptographic parameters and hardware pipelines. We organize one bootstrappable and two swift clusters into one cluster affiliation, and present a scheduling scheme that provides sufficient acceleration for deep FHE workloads by utilizing all the affiliations, while improving parallelism for shallow FHE workloads by assigning one shallow workload per affiliation and dynamically decomposing the bootstrappable cluster into multiple swift pipelines to accelerate the assigned workload. We further show that these two types of clusters can share valuable on-chip memory, improving performance without significant resource consumption. We implement FLASH-FHE with RTL and synthesize it using both 7nm and 14/12nm technology nodes, and our experiment results demonstrate that FLASH-FHE achieves an average performance improvement of $1.4\times$ and $11.2\times$ compared to state-of-the-art FHE accelerators CraterLake and F1 for deep workloads, while delivering up to $8.0\times$ speedup for shallow workloads due to its heterogeneous architecture.

==> algorithms/design/key-switching.tex <==
\begin{algorithm}[H]
\footnotesize
\renewcommand{\algorithmiccomment}[1]{\hfill $\triangleright$ #1}
\newcommand{\GreenColorLine}[1]{
\hspace{-0.03\linewidth}\colorbox{green!30}{\makebox[0.99\linewidth][l]{#1}}}
\newcommand{\RedColorLine}[1]{
\hspace{-0.03\linewidth}\colorbox{red!30}{\makebox[0.99\linewidth][l]{#1}}}
\caption{Example step in key-switching for compound operation opimization}
\label{alg:compound_op_opimization}
\begin{algorithmic}[1]
\FORALL{$i=0, 1, ..., l$}
\STATE $c_2\_iNTT[i]=\textbf{INTT}(c_2[i])$
\ENDFOR
\FORALL[Outer Loop]{$i=0, 1, ..., l+1$} \label{alg:compound_op_opimization_outer_loop}
\IF{$i=l+1$}
\STATE $index= L+1$
\ELSE
\STATE $index=i$
\ENDIF
\FORALL[Inner Loop]{$j=0, 1, ..., l$} \label{alg:compound_op_opimization_inner_loop}
\IF{$i=j$}
\STATE $operand=c_2[j]$
\ELSE
\STATE $operand=\textbf{NTT}(c_2\_iNTT[j]) \mod q_{index}$
\STATE $ans_0[i]=ans_0[i]+operand \cdot $$swk_0[j][index] \mod q_{index}$ \label{alg:compound_op_opimization_overhead_1}
\STATE $ans_1[i]=ans_1[i]+operand \cdot $$swk_1[j][index] \mod q_{index}$ \label{alg:compound_op_opimization_overhead_2}
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> sections/analysis_archive.tex <==
\section{Analysis on Existing Architectures}
\label{sec:analysis}

\input{figures/fig-naive-group-arch}

To answer this question, in this paper, we first perform extensive analysises over the existing \group and \grid architectures to establish a \emph{quantitative} connection between these designs and \highlight{both their performance and resource consumption.}

As we have mentioned in \secref{sec:background}, the key-switching is a fundamental operation in homomorphic multiplication and bootstrapping, which takes $>XX\%$ execution time~\cite{}. One important and commonly-used operation in key-switching is the BConv operation. However, as shown in Equation~\ref{eq:bconv}, BConv consists of modulus conversions and thus cannot be directly performed on polynomials in the NTT form~(the polynomials are converted into the NTT form as possible to accelerate the multiplication operation). We have to perform an iNTT operation first, then BConv and finally a NTT operation to convert the polynomial back into the NTT form. Thus, the iNTT $\rightarrow$ BConv $\rightarrow$ NTT pipeline is very common in FHE schemes~\cite{bts,craterlake}, and it takes $>XX\%$ overall execution time. \highlight{Considering the hardware resource consumption, in our analysis, we mainly focus on the number of 32-bit multipliers (\mul) required to implement the design. TODO: What about the memory? In common knowledge, the memory components should take the majority resources.}

In this section, we will first introduce the NTT/iNTT and BConv pipeline of the \group and \grid architectures in \secref{sec:group_arch} and \secref{sec:grid_arch}, respectively. Furthermore, we will combine these pipelines into a complete performance model \highlight{of iNTT $\rightarrow$ BConv $\rightarrow$ NTT pipeline} in \secref{sec:analysis_combine}. However, before digging into the details of the two architectures, we will first introduce a \emph{na\"ive} NTT/iNTT implementation.

%As introduced in \secref{sec:background_fhe_optimization}, the NTT/iNTT module can optimize polynomial multiplication, thus, is fundamental in various FHE operations, \eg, ciphertext multiplication, key-switching, bootstrapping, \etc. 
\figref{fig:naive_arch} shows a Na\"ive NTT/iNTT pipeline implementation supporting polynomial degree $N=8$, which is also referred to as an $N$-point NTT. The pipeline takes eight inputs and the number of stages in the pipeline is $\log N = \log_2 8 = 3$. Thus the total pipeline execution time is $\log N \cdot T_{butterfly}$, where $T_{butterfly}$ is the execution time of one butterfly operation. \highlight{In our paper, we use hardware cycle to denote the execution time since the  computation time can be calculated if given the hardware frequency. As an initial step, we perform analysis to obtain the hardware cycles needed for one butterfly operation, $T_{\rm butterfly}$, is 22~(Please see \appref{} for detailed analysis on $T_{\rm butterfly}$).}


The na\"ive NTT/iNTT pipeline can achieve very high performance with a considerable number of polynomials in FHE operations. However, the major drawback is that it consumes too many resources, \ie, $N/2 \cdot \log N$ butterfly units, which is not practical in real-world implementations. Moreover, the generality of such na\"ive implementation is also limited, leading to underutilization of computing hardware resources.

To optimize the aforementioned resource consumption, the NTT/iNTT pipeline can be decomposed into multiple smaller ones based on the four-step FFT/NTT algorithm. In the four-step FFT/NTT scheme, the $N$ input numbers can be represented as a~$\boldsymbol{N}=R \times C$ matrix since $N$ is typically a power of two in FHE. The algorithm can be executed using the combination of row NTTs as described in the following workflow:

\begin{icompact}
\item[i.] Transpose the input matrix into a $C \times R$ matrix. Perform a na\"ive $R$-point NTT on each row of the input matrix and these NTT results are aggregated into a new matrix $\boldsymbol{A'}$ with a shape of $C \times R$.
\item[ii.] Generate a $C \times R$ twisting factor matrix $\boldsymbol{F}$ and perform dyadic multiplication between matrix $\boldsymbol{A'}$ and matrix $\boldsymbol{F}$. Let matrix $\boldsymbol{A''}$ denote the multiplication result.
\item[iii.] Transpose the matrix $\boldsymbol{A''}$ to obtain a $\boldsymbol{A'''}=R \times C$ matrix.
\item[iv.] Perform a na\"ive $C$-point NTT on each row of the matrix $\boldsymbol{A'''}$ and get the matrix aggregating the NTT results. Transpose the result matrix and get the final result with the shape of $C \times R$.
\end{icompact}

In hardware implementations, since the storage order of the coefficients does not influence the execution of element-wise polynomial operations, the first and last transposes can usually be saved by storing the matrices in column-major order.

Both the \group and \grid architectures leverage the four-step FFT/NTT algorithm \highlight{as a core optimization strategy} to improve data parallelism and reduce resource consumption in NTT/iNTT pipelines with distinct designs.

\tabref{tab:notations} shows the notions used in the following sections.

\subsection{Group Architecture}

\label{sec:group_arch}

The \group architecture for accelerating FHE schemes \highlight{was proposed by CraterLake~\cite{craterlake} and used by ARK~\cite{ark}, \etc.}
%has been widely adopted by recent works such as CraterLake~\cite{craterlake}, ARK~\cite{ark}, \etc. 
%For easy understanding, 
In this section we will base our analysis on the physical design of CraterLake, but our analysis can generalize to other FHE accelerators that leverage the \group architecture as their core physical designs.

\figref{fig:group_arch}~(left part) shows the physical design of the \group architecture.
%CraterLake allocates eight physical computation groups, \ie, group engines.
We use $G$ to denote the number of computation groups (\ie, group engines) in the architecture.
Each group engine contains a $R$-point NTT/iNTT pipeline~(right-up part of \figref{fig:group_arch}). The workflow of the \group architecture mainly follows the four-step FTT/NTT algorithm~(right-bottom part of \figref{fig:group_arch}). 

\highlight{Another design choice adopted by the \group architecture of CraterLake is to use a \highlight{parallel} BConv module. As shown in \figref{fig:parallel_bconv}, the parallel BConv consists of a broadcast module and $\alpha$ independent basis converters, each of which calculates element-wise modular multiplications and summation with different moduli concurrently. Every polynomial fed to the architecture is broadcasted to all the basis converters for the calculations. The BConv unit consumes a total number of $G \cdot R \cdot L$ \mul{}s in the entire group architecture.}

%Next, we will evaluate the performance of NTT/iNTT pipeline and BConv module, respectively.

\parab{NTT/iNTT Pipeline:} 
%Similar to previous analysis, we still use hardware cycle to evaluate the pipeline performance. 
\highlight{Since RNS decomposition is used to decompose a polynomial with large coefficients into $l$ polynomials with much smaller coefficients, which can be fit in hardware.} Thus, in quantifying the performance of the pipeline, 
%we will consider the RNS decomposition in our analysis, \ie, 
the number of polynomials to be processed should times $l$. 

Based the workflow of \group architecture, as shown in \figref{fig:group_arch}, the total cycles $T$ needed for the pipeline can be calculated using the following equation.

\begin{equation}
	T = T_{\rm D1} + T_{\rm twisting\_factor} + T_{\rm transpose} + T_{\rm D2}
\end{equation}

\highlight{
The $T_{\rm twisting\_factor}$ denotes the cycles needed to perform a dyadic multiplication between matrix $\boldsymbol{A'}$ and matrix $\boldsymbol{F}$ while the $T_{\rm transpose}$ denotes the time to perform a transpose. In our paper, we perform analysis on their corresponding circuits to obtain the hardware cycles needed and we have $T_{\rm twisting\_factor}=17$ and $T_{\rm transpose} =$ \highlight{$???$}. Interested readers can refer to \appref{} for more details.}
Therefore, to obtain the overall performance of NTT/iNTT pipeline, the remaining part is to calculate the cycles consumed by these group engines when performing NTT/iNTT operations on the first and second dimension of the matrix, respectively, \ie, $T_{\rm D1}$ and $T_{\rm D2}$.

When estimating the $T_{\rm D1}$ and $T_{\rm D2}$, we have one reasonable assumption that the group engine is fully pipelined, \ie, there is only one cycle delay when processing two consecutive $R$-point or $C$-point NTTs. Then, as shown in \figref{fig:group_arch}, the execution time of $T_{\rm D1}$ contains two parts. The first part is the execution cycle of $R$-point NTT, which equals the number of stages times the cycle per stage: $\log R \cdot T_{\rm butterfly}$. The second part is the delayed cycles used to pipeline all polynomials, which equals the number of all polynomials to be processed. Since CraterLake adopts eight parallel group engines~\highlight{TODO: Why do we mention eight here?}, each with a $R$-point NTT/iNTT pipeline, the computation of an $N$-point NTT is decomposed into $N/R$ $R$-point NTTs and each group engine has $N/(R \cdot G)$ $R$-point NTTs to be processed. Moreover, considering the RNS decomposition used in the FHE scheme, each $N$-point NTT should be performed on each of the $L$ polynomials. Thus, the total number of $R$-point NTTs to be processed per group engine equals $N \cdot L/(R \cdot G)$. Finally, we obtain $T_{\rm D1} = \log R \cdot T_{\rm butterfly} + N \cdot L/(R \cdot G)$.

To estimate the $T_{\rm D2}$, we can use a similar method. Since CraterLake supports a maximum $N=65536$, and $N$ is a power of $2$. $R$ is larger than $N/R$, and $R/(N/R)$ should yield a integer. As a result, we can execute $R/(N/R)$ $C$-point NTTs simultaneously with a single $R$-point NTT pipeline. As a result, the execution time of the pipeline is $\log(N/R) \cdot T_{\rm butterfly}$ cycles, and the total number of $N/R$-point NTTs to be processed per group engine equals to $R \cdot L/(R/(N/R))/G = N\cdot L/(R \cdot G) $. Thus we can obtain $T_{D2} = \log (N/R) \cdot T_{\rm butterfly} + N\cdot L/(R \cdot G)$.

%Summing up the execution times of all four parts leads to an estimation of the absolute performance. Then, we will demonstrate the resource used to implement the \group NTT/iNTT architecture to inform the performance per resource metric. 

\highlight{For the resource consumption,} in each group, the $R$-point NTT pipeline consists of $\log R$ sequential computation stages and $R/2$ \mul{}s are required for the $R/2$ parallel butterflies in each stage. As a result, the group architecture needs a total number of $(G\cdot R \cdot \log R) / 2$ \mul{}s for the NTT/iNTT module.


\parab{Parallel BConv:} To analyze the performance of the BConv unit, we assume that all the input data of BConv is already cached on the chip so that the execution of BConv is fully pipelined. The length of the pipeline is the time required for an addition and a multiplication, which equals 18 cycles. The total number of input polynomials in a single BConv operation is $L$ and each polynomial contains $N$ coefficients. As there are $G$ groups in the architecture and each calculation group consumes $R$ coefficients every cycle, the entire architecture can consume $G\cdot L \cdot R$ coefficients each cycle during Bconv and finishes reading all the input data in $N \cdot L/ (G\cdot R)$ cycles. Therefore, the execution time of the fully pipelined parallel BConv unit is $N \cdot L/ (G\cdot R) + 18$.

The resource consumption of the parallel BConv unit is significant as it requires $\alpha$ parallel basis converters in each group. Each converter requires $R$ \mul{}s to consume $R$ coefficients from the broadcast module every cycle. Thus, the entire parallel BConv needs $G\cdot \alpha \cdot R$ \mul{}s for the basis conversion operation.

\subsection{Grid Architecture}

\label{sec:grid_arch}

The \grid architecture is \highlight{proposed by} BTS~\cite{bts}, and its physical design is to allocate various computation engines~(\eg, $32 \times 64$ engines in BTS) on a grid, as shown in \figref{fig:grid_arch}~(left part). Each engine contains a two-point NTT pipeline. All engines are connected using a special network: crossbar interconnection~\cite{}. The \grid architecture further decomposes the NTT/iNTT pipeline into a three-dimension matrix multiplication: $\boldsymbol{N}= T \times R \times C$, and the two data transposes occur vertically and horizontally respectively in the grid to achieve global data synchronization, which could fully utilize the cross-bar structure. The $R$ equals the number of rows of engines whereas $C$ equals the number of columns.

Moreover, the \grid architecture uses a sequential BConv module. Different from the design in the group architecture, each grid in the grid architecture contains a sequential BConv unit that reuses the same basis converter rather than $L$ independent ones, as demonstrated in \figref{fig:sequential_bconv}. The basis converter in the \grid architecture mainly consists of a modular multiply-accumulate unit, including $l_{\rm{sub}}$ \mul{}s and $l_{\rm{sub}} - 1$ adders. The number $l_{\rm{sub}}$ is an integral power of two and is set to reduce the waiting \highlight{time} between \highlight{iNTT} and BConv operations.


\input{figures/fig-grid-arch}

\parab{NTT/iNTT Pipeline:} The workflow of the \grid architecture is shown on the right part of \figref{fig:grid_arch}: 1) each engine performs a $T$-point NTT, which is independent with each other; 2) all engines perform a vertical data synchronization to transpose the input data, and further perform a $R$-point NTT on each column of engines; 3) all engines perform a horizontal data synchronization to transpose the input data, and further perform a $C$-point NTT on each row of engines. Thus the total cycles $T$ needed for the pipeline is:

\begin{equation}
\begin{split}
T = &\quad T_{\rm D1} + T_{\rm twisting\_factor} + T_{\rm v\_sync} + \\
&\quad T_{\rm D2} + T_{\rm twisting\_factor} + T_{\rm h\_sync} + T_{\rm D3}
\end{split}
\end{equation}

The synchronization, $T_{\rm v\_sync}$ and $T_{\rm h\_sync}$, both take \highlight{???} cycles, and more details are presented in \appref{}. The $T_{\rm twisting\_factor}=17$ cycles as mentioned previously. Thus, to quantify the overall NTT/iNTT pipeline performance of the \grid architecture, we have to obtain the performance of $T_{\rm D1}$, $T_{\rm D2}$, and $T_{\rm D3}$. Similar to our analysis in \secref{sec:group_arch}, we assume all engines are fully pipelined, and the RNS decomposition yields $l$ times polynomials.

Let's first consider the $T_{\rm D1}$, which equals the time that all engines perform a $T$-point NTT, where $T = N/(R \cdot C)$. Since each engine could only process a two-pint NTT, processing $T$-point NTT requires $\log \frac{N}{C \cdot R}$ stages.
%Note here we do not use $\log \frac{N}{C \cdot R \cdot 2}$ since reading from the same input requires 2 cycles to avoid reading collision.
The computations in different stages can hardly be pipelined due to their data dependency, thus $T_{D1} = \log \frac{N}{C \cdot R} \cdot T_{\rm stage}$ in our analysis, where $T_{\rm stage}$ denotes the cycles needed to complete one stage. Similarly to \group architecture, the total cycles of $T_{\rm stage}$ contain two parts: 1) the cycles used for two-point NTT pipeline execution, which equals $T_{\rm butterfly}$ and 2) the delayed cycles to process all NTT computations, as shown in \figref{fig:grid_arch}~(up-right part). In each stage, there are $L \cdot N / (2 \cdot C\cdot R)$ two-point NTTs to be processed. Therefore, $T_{\rm stage} = T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R)$. Thus the total cycles needed to complete the first dimension computation $T_{\rm D1} = \log \frac{N}{C \cdot R} \cdot (T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R))$.

The calculation of $T_{\rm D2}$ and $T_{\rm D3}$ is similar to $T_{\rm D1}$. The difference is that in the second dimension, the number of stages is $\log R$ while in the third dimension, the number of stages is $\log C$. Thus we have $T_{\rm D2} = \log R \cdot (T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R))$ and $T_{\rm D3} = \log C \cdot (T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R))$.

Next, we will estimate the resources needed to implement the \grid NTT/iNTT architecture. \highlight{In each grid, there's only one butterfly unit which needs one \mul. Thus, the entire architecture requires $R\cdot C$ \mul{}s for the NTT/iNTT calculation.}

\parab{Sequential BConv:} Similar to the analysis before, we assume that all the input data is ready and the converter is fully pipelined. The basis converter reads $l_{\rm{sub}}$ coefficients each cycle and performs basis conversion with a certain modulus which requires an execution time of $17 + \log l_{\rm{sub}} + 1$ cycles to go through the pipeline. As we analyzed in \S\ref{sec:group_arch}, the number of input coefficients is $N\cdot L$ and each data should be reused by $L$ times for the calculation with different moduli, leading to a total number of input data of the converter pipeline is $N\cdot L^2$. Therefore, the total execution time for the sequential BConv is $N \cdot L^2 + 17 + \log l_{\rm{sub}}$.

By sacrificing a certain amount of performance, sequential BConv significantly reduces the amount of resources required compared to parallel BConv. In the grid architecture, we only have $l_{\rm sub}$ \mul{}s in each grid, leading to a total amount of $R\cdot C \cdot l_{\rm sub}$ \mul{}s in the entire architecture.

\subsection{Quantitative Performance Model}
\label{sec:analysis_combine}

In this section, we will combine the components discussed in \secref{sec:group_arch} and \secref{sec:grid_arch} to inform a complete performance model to quantify the practical efficiency of these existing architectures. \highlight{We will first introduce the performance model and then explain the advantages and disadvantages of the \group and \grid architectures based on the performance model.}

\input{figures/fig-ks-pipeline}

\subsubsection{Performance Model}

\label{sec:analysis_performance_model}

\figref{fig:ks_pipeline} shows the aforementioned iNTT $\rightarrow$ BConv $\rightarrow$ NTT pipeline. In this paper, we consider that both the \group and \grid architecture choose to pipeline BConv with iNTT~\footnote{The original paper of \grid architecture has pointed out that it pipelines BConv with iNTT~\cite{bts}. However, for \group architecture, readers can consult \appref{} to see why we consider that it also pipelines BConv with iNTT.}. Thus, the overall pipeline execution time equals the sum of one NTT pipeline time, $T_2$, and the total execution time of the iNTT and BConv, $T_1$. Since we have obtained the NTT time in the previous sections, the key is to obtain the $T_1$.

To obtain $T_1$, we observe that the BConv can only be pipelined with the last dimension computation, \ie, the D2 with the \group architecture, and the D3 with the \grid architecture, as shown in \figref{fig:ks_pipeline}~(bottom part). Therefore, we can use a similar calculation method as \secref{sec:group_arch} and \secref{sec:grid_arch} to evaluate $T_1$. It is worth noting that we assume the parallel BConv consumes less execution time than \group iNTT while the sequential BConv is slower than \grid iNTT since $l_{\rm sub}$ is usually selected as a small integer. Finally, we can calculate $T_1$ with the following \equref{eq:group_arch_model} for the \group architecture.

\begin{equation}
\begin{split}
	T_1 = 
		&\quad \log R \cdot T_{\rm butterfly} + N \cdot L/(R \cdot G) + \\
		&\quad T_{\rm twisting\_factor} + T_{\rm transpose} + \\
		&\quad \log \frac{N}{R} \cdot T_{\rm butterfly} + N \cdot L/ (R\cdot G) + 18
\end{split}
\label{eq:group_arch_model}
\end{equation}

Similarly, we can obtain the $T_1$ with the following \equref{eq:grid_arch_model} for the \grid architecture.

\begin{equation}
\begin{split}
	T_1 = 
		&\quad \log \frac{N}{C \cdot R} \cdot (T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R)) + \\
		&\quad T_{\rm twisting\_factor} + T_{\rm v\_sync} + \\
		&\quad \log R \cdot (T_{\rm butterfly} + L \cdot N / (2 \cdot C\cdot R)) + \\
		&\quad T_{\rm twisting\_factor} + T_{\rm h\_sync} + \\
		&\quad N \cdot L \cdot l/(C \cdot R \cdot l_{\rm{sub}}) + \log l_{\rm sub} + 17 + \\
		&\quad \log C \cdot (N/(2\cdot C \cdot R) \cdot l_{\rm{sub}}+T_{\rm butterfly})
\end{split}
\label{eq:grid_arch_model}
\end{equation}

From the previous analysis, we can also estimate the total resource consumption of \group and \grid architecture including NTT/iNTT and BConv, which requires $\left( G\cdot R \cdot \left(\alpha + \frac{\log R}{2}\right) \right) $ and $R\cdot C\cdot (1+l_{\rm sub})$ \mul{}s, respectively.

\subsubsection{Analysis Results}
\label{sec:analysis_results}

\input{figures/analysis/fig-analysis-performance}

Based on the performance model in \secref{sec:analysis_performance_model}, we present the following key results, and leave more results in \appref{} for interested readers.

First, we show the absolute performance achieved by both \group and \grid architectures. Then we consider their resource consumption to demonstrate performance per \mul{}. \highlight{Here, we use the throughput~(Thr.) of pipeline to denote the performance, which is calculated as $f / T$, where $f$ denotes the frequency, and $T$ denotes the cycles needed. Here, we set $f=1$Ghz\footnote{\highlight{The original paper of \group architecture reports that they use 1Ghz hardware frequency~\cite{craterlake}. However, the original paper of \grid uses a slightly higher value: 1.2Ghz~\cite{bts}. Hereby, we use 1Ghz for a practical and fair comparison}.}}
Meanwhile, we let \highlight{$L=16$, XXX, as a typical setting.} 

\figref{fig:analysis_results} shows our analysis results. First, from \figref{fig:arch_abs_performance}, we can observe that the \group architecture can achieve much lower pipeline execution time~(up to $3.1\times$ when $l=16$) compared to \grid architecture, which could further lead to a much higher pipeline throughput. The reason is that the NTT pipeline in \grid architecture takes much longer time to execute, thus degrading the overall performance. Moreover, the parallel BConv module is also faster than sequential BConv. Second, \figref{fig:arch_performance_per_resource} shows that considering the pipeline throughput per \mul{}, \grid architecture can achieve better results than \group. For example, when $l=1$, the throughput per \mul{} of the \grid architecture is $2.6\times$ of the \group architecture. The reason is that the parallel BConv module consumes too many resources, which is underutilized when $l$ is small.

\parab{Summary:} Existing architectures, \ie, \group and \grid architecture, either suffer from degraded absolute performance or sub-optimal performance per resource, thus failing to achieve our practical efficiency goal. We are asking a fundamental question: is there a more practical FHE accelerator that could achieve practical efficiency?


==> tables/evaluation/tab-performance-12nm.tex <==
\begin{table*}
\small
\centering
\begin{threeparttable}
\begin{tabularx}{\linewidth}{Xccccccccc}
\toprule
\multirow{2}{*}{Execution Time (ms) on} & \multirow{2}{*}{\sys} & \multirow{2}{*}{CraterLake} & \multirow{2}{*}{F1+} & \multirow{2}{*}{CPU} & \multicolumn{2}{c}{vs. CraterLake} & \multicolumn{2}{c}{vs. F1+} & \multirow{2}{*}{vs. CPU} \\
\cline{6-9}
& & & & & Abs. & Rel. & Abs. & Rel. & \\
\midrule
%Unpacked Bootstrapping & & & & & & & & \\
CIFAR Unencryp. Wghts. & 9.60 & 50.50 & 94.10 & 187 s & 5.26$\times$ & 4.90$\times$ & 9.80$\times$ & 12.29$\times$ & 19,479$\times$ \\
MNIST Unencryp. Wghts. & 0.18\tnote{a} & 0.14 & 0.13 & 561 & 0.77$\times$ & 0.72$\times$ & 0.72$\times$ & 0.90$\times$ & 3,099$\times$ \\
MNIST Encryp. Wghts. & 0.19 & 0.24 & 0.22 & 1,369 & 1.27$\times$ & 1.18$\times$ & 1.16$\times$ & 1.46$\times$ & 7,243$\times$ \\
%\midrule
%\multicolumn{7}{l}{\textbf{Average Speedup (Geometric Mean) for Shallow FHE Workloads}} &  & ? & ? & ? & ? & ? \\
\midrule
Packed Bootstrapping & 2.64 & 6.33 & 58.30 & 17.2 s & 2.40$\times$ & 2.23$\times$ & 22.09$\times$ & 27.70$\times$ & 6,516$\times$ \\
ResNet-20 & 63.27 & 321.26 & 2,693 & 23 min & 5.08$\times$ & 4.73$\times$ & 42.56$\times$ & 53.38$\times$& 21,811$\times$  \\
Logistic Regression~(32 iteration) & 34.16 & 121.91 & 639.00 & 356 s & 3.57$\times$ & 3.32$\times$ & 18.70$\times$ & 23.46$\times$ & 10,420$\times$ \\
LSTM & 160.14 & 223.56 & 2,573 & 859 s & 1.40$\times$ & 1.30$\times$ & 16.07$\times$ & 20.15$\times$ & 5,364$\times$ \\
%\midrule
\midrule
\multicolumn{4}{l}{\textbf{Average Speedup (Geometric Mean) for Mixed FHE Workloads}}  &  & \textbf{2.27$\times$} & \textbf{2.12$\times$} & \textbf{8.11$\times$} & \textbf{10.18$\times$} & \textbf{8,598$\times$} \\
\bottomrule
\end{tabularx}
\begin{tablenotes}
\item[a] \sys uses $L=6$ in this case while F1 and CraterLake use $L=4$. This discrepancy arises because we encountered difficulties in successfully running this particular case with $L=4$.
\end{tablenotes}
\caption{[14/12nm Technology Node] Performance of \sys with three shallow and four deep FHE applications. The table compares the absolute performance (Abs.) and relative performance (Rel.) of \sys (synthesized with the 14nm technology node) with CraterLake and F1+, which all use the 14/12nm technology node. We also compare \sys with an AMD Ryzen Threadripper PRO 3975WX 32-core, 64-thread CPU. The batch size of Logistic Regression is 256.}
\label{tab:eval-performance-12nm}
\end{threeparttable}
\end{table*}


==> tables/evaluation/tab-performance-7nm.tex <==
\begin{table*}
\small
\centering
\begin{tabularx}{\linewidth}{l Y Y Y Y Y Y Y}
\toprule
\multirow{2}{*}{Execution Time (ms) on} & \multirow{2}{*}{\sys} & \multirow{2}{*}{ARK} & \multirow{2}{*}{SHARP} & \multicolumn{2}{c}{v.s. ARK} & \multicolumn{2}{c}{v.s. SHARP}\\
& & & & Abs. & Rel. & Abs. & Rel. \\
\midrule
ResNet-20 & 63.27 & 125.00 & 99.00 & 1.98$\times$ & 4.73$\times$ & 1.56$\times$ & 1.60$\times$ \\
Logistic Regression~(one iteration) & 1.19 & 7.42 & 2.53 & 6.24$\times$ & 15.83$\times$ & 2.13$\times$ & 2.31$\times$ \\
\bottomrule
\end{tabularx}
\caption{[7nm Technology Node] Performance of \sys compared to ARK and SHARP. The batch size of Logistic Regression is 1024. The table compares the absolute performance (Abs.) and relative performance (Rel.).}
\label{tab:eval-performance-7nm}
\end{table*}
